Weakly Supervised Semantic Segmentation using Web-Crawled Videos

We propose a novel algorithm for weakly supervised semantic segmentation based on image-level class labels only. In weakly supervised setting, it is commonly observed that trained model overly focuses on discriminative parts rather than the entire object area. Our goal is to overcome this limitation with no additional human intervention by retrieving videos relevant to target class labels from web repository, and generating segmentation labels from the retrieved videos to simulate strong supervision for semantic segmentation. During this process, we take advantage of image classification with discriminative localization technique to reject false alarms in retrieved videos and identify relevant spatio-temporal volumes within retrieved videos. Although the entire procedure does not require any additional supervision, the segmentation annotations obtained from videos are sufficiently strong to learn a model for semantic segmentation. The proposed algorithm substantially outperforms existing methods based on the same level of supervision and is even as competitive as the approaches relying on extra annotations.

==> overview.tex <==
% !TEX root = cvpr2017_seg.tex
\section{Overview}
\label{sec:overview}

%
\begin{figure*}[!t]
\centering
\vspace{2cm}
FIGURE DESCRIBING OVERALL FRAMEWORK OF THE PROPOSED APPROACH
\vspace{2cm}
\caption{
Overall framework of the proposed algorithm.
Our algorithm first learns a model for classification and localization from a set of weakly annotated images (Section~\ref{sec:attention_classification}). 
The learned model is used to eliminate noisy frames and generate coarse localization maps in weakly-annotated videos, where the per-pixel segmentation masks are obtained by solving a graph-based optimization problem (Section~\ref{sec:video_segmentation}).
%The obtained segmentations are used to learn a decoder that takes attention map as an input and produces binary segmentation mask as an output. 
% The obtained segmentations are served as ground-truth data to train a model, which is used to generate semantic segmentation on still images (Section~\ref{sec:decoder}). 
The obtained segmentations are served as annotations to train a model for semantic segmentation in still image (Section~\ref{sec:decoder}). 
}
\label{fig:overview}
\end{figure*}
%


%\ifdefined\paratitle {\color{blue} 
%[Definition of problem setting: dataset] \\
%} \fi

%The objective of this paper is to exploit two sets of heterogeneous data--weakly-annotated images and videos--to improve weakly-supervised semantic segmentation on still images.
%The objective of this paper is to learn a model for weakly-supervised semantic segmentation by exploiting videos collected from web in addition to weakly-annotated images.
%The objective of this paper is to learn a model for semantic segmentation using two sets of heterogeneous data--weakly-annotated images and videos.
%The objective of this paper is to learn a model for semantic segmentation by exploiting complementary benefits of two heterogeneous data--weakly-annotated images and videos.

%The objective of this paper is to improve a weakly-supervised semantic segmentation by exploiting complementary benefits of two heterogeneous data--images and videos.
\iffalse
The objective of this paper is to improve a weakly-supervised semantic segmentation using two heterogeneous data--images and videos.
Let $\I=\{(\x_k, \y_k)\}$ denotes a set of weakly-annotated images, where $\x_k$ is an image and $\y_k\in\{0,1\}^L$ is an indicator vector for $L$ categories. 
Then we collect a set of videos from web $\V=\{(\X_k, \y_k)\}$, where $\X_k=\{\x_1,...,\x_{N_k}\}$ is a video composed of $N_k$ frames.
\fi
%Let $\I$ and $\V$ denote set of images and videos, respectively, where each element of the sets corresponds to images and videos associated with class labels. 
Let $\I$ and $\V$ denote datasets of weakly annotated images and videos, respectively. 
%We assume that each element in $\I$ is an image associated with image-level class label annotated by human, and the ones in $\V$ is a video collected from web associated with a class label used as search keyword.
%Each element in $\I$ is a tuple composed of an image and class labels obtained by human annotator, and similarly for $\V$ where each element is composed of a video collected from web and a class label used as search keyword for collected video. 
Each element in $\I$ is a tuple composed of an image and class labels given by human annotator, and similarly, an element in $\V$ is a pair of a video collected from the Web and a class label used as a search keyword during data collection. 
%Each element in $\I$ is an image associated with class labels given by human annotator, and similarly for $\V$ which is a video collected from web and a class label used as a search keyword during data collection. 
Our objective is to learn a model for semantic segmentation using complementary benefits of these heterogeneous data.
%Given these two sets of data, our objective is to learn a model for semantic segmentation.

The overall pipeline of the proposed framework is described in Figure~\ref{fig:overview}. 
We employ a decoupled deep encoder-decoder architecture from \cite{transfernet} as our model for semantic segmentation with modification on attention mechanism. 
In this architecture, the attention model identifies salient parts of an image for each category, where the decoder generates dense binary segmentation mask of each focused object using coarse attention map as an input.
To exploit complementary benefits of images and videos, we train each component of the model using different sets of data by following procedures:%as summarized below: 

\iffalse
Things to discuss:
model architecture.
why this architecture is beneficial for this particular setting
why we separately train different components of the model with different annotations
\fi
%
\begin{itemize}
\item 
Given a set of weakly-annotated images $\I$, we train recognition and attention models under classification objective (Section~\ref{sec:attention_classification}).
\item 
%Then we perform segmentation on a set of weakly-annotated videos $\V$ to generate segmentation masks of object by optimizing spatio-temporal graphical model (Section~\ref{sec:video_segmentation}).
%In this stage, we employ attention model trained on images to reduce noises in videos.
We apply the learned recognition and attention models to videos to filter out frames irrelevant to class label and generate coarse attention maps of target object in every remaining frames, respectively.
Then spatio-temporal object segmentations are obtained from videos by optimizing graphical model (Section~\ref{sec:video_segmentation}).
\item 
Using obtained segmentation labels from videos, we train a decoder that maps an coarse attention map to dense binary segmentation (Section~\ref{sec:decoder}).
Then semantic segmentation on still images is performed by applying a learned network. 
\end{itemize}
%



\iffalse
Let $\I=\{(\x_k, \y_k)\}$ and $\V=\{(\X_k, \y_k)\}$ denote sets of weakly-annotated images and videos, respectively, where $\x_k$ is an image, $\X_k=\{\x_1,...,\x_{N_k}\}$ is a video composed of $N_k$ frames, and $\y_k\in\{0,1\}^L$ is an indicator vector over $L$ categories. 
Our objective is to improve a weakly-supervised semantic segmentation by exploiting complementary benefits of two heterogeneous data--images and videos.
\fi
%Then we collect a set of videos from web and construct a set of weakly-labeld videos $\V=\{(\X_k, \y_k)\}_{k=1}^{N_V}$, where $\X_k=\{\x_1,...,\x_{N_k}\}$ is a video composed of $N_k$ frames and $\y_k$ is a label used to collect a video $\X_k$.


\iffalse
The proposed model exploits complementary benefits from both images and videos as follow.
First, weakly-labeled labels in images are clean since it is obtained by user, and useful to learn recognition model to identify presence of object class, and attention model to identify coarse spatial configuration of objects.
Since the attention model favors only discriminative parts of object due to discriminative training, however, it is difficult to figure out entire object areas or precise shape boundaries.
On the other hand, videos contain motion and temporal context, which are useful to infer object shape.
However, the video data is noisy since it is automatically collected through web search, and loose association between labels and frames.
By employing recognition model and attention model, we can resolve uncertainties in weakly-annotated videos in both spatial and temporal domain.
\fi

%The employed architecture based on attention is well-suited for this particular setting.
 





